From Asset Flow to Status, Action and Intention Discovery: Early Malice Detection in Cryptocurrency

Cryptocurrency has been subject to illicit activities probably more often than traditional financial assets due to the pseudo-anonymous nature of its transacting entities. An ideal detection model is expected to achieve all three critical properties of (I) early detection, (II) good interpretability, and (III) versatility for various illicit activities. However, existing solutions cannot meet all these requirements, as most of them heavily rely on deep learning without interpretability and are only available for retrospective analysis of a specific illicit type. To tackle all these challenges, we propose Intention-Monitor for early malice detection in Bitcoin (BTC), where the on-chain record data for a certain address are much scarcer than other cryptocurrency platforms. We first define asset transfer paths with the Decision-Tree based feature Selection and Complement (DT-SC) to build different feature sets for different malice types. Then, the Status/Action Proposal Module (S/A-PM) and the Intention-VAE module generate the status, action, intent-snippet, and hidden intent-snippet embedding. With all these modules, our model is highly interpretable and can detect various illegal activities. Moreover, well-designed loss functions further enhance the prediction speed and model's interpretability. Extensive experiments on three real-world datasets demonstrate that our proposed algorithm outperforms the state-of-the-art methods. Furthermore, additional case studies justify our model can not only explain existing illicit patterns but can also find new suspicious characters.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> section/5_5_segments_and_status_generation.tex <==
\input{table/split_compare}
% Input features shouldn't change significantly over time for a decision tree. 
% If features vary dramatically in different time slices, 
% the model can't learn a stable distribution and will fail to predict the test data. 
%
% Therefore, 
To prove the necessity of segment splitting,  
we compare the performance model with and without splitting processing.
Besides, instead of only splitting based on the features' change ratio, 
we also analyze the performance of the extra two splitting methods.


The first splitting method \textbf{M1} is the same as the descriptions in Sec.~\ref{sec:DT_SA_with_SPM}. 
%
Besides, many malicious activities are executed with a modus operandi attack system. 
% To avoid attracting unnecessary attention, 
They are set to operate according to the Fibonacci sequence or uniform time series. 
Thus, the second \textbf{M2} and the third \textbf{M3} splitting methods are Fibonacci sequence and uniform splitting (segmented every ten hours). 
Model without splitting is denoted as \textbf{w/o}.
\textbf{+X} stands for combing splitting method \textbf{X} with previous splitting scheme.
The performance is calculated as the average of $10$ independent experiments.

Considering malicious addresses are inactive in many segments, 
the models can hardly predict correctly during these segments.
In this case, comparing $F1^C$ and $F1^E$ is unfair. 
Meanwhile, we expect the models to capture discriminative information in early segments to make accurate predictions earlier. 
Therefore, we use $F1^H$, $T^H$, and $\Delta$ to evaluate each splitting method.
%
$F1^H$ refers to the mean value of the highest $F1$ scores over $10$ independent trials. 
$T^H$ refers to the average time to reach the highest $F1$ in these $10$ trials (the highest $F1$ for each experiment is not necessarily $F1^H$).
%
For $\Delta$, take \textbf{w/o} and \textbf{M1} as an example.
We refer time $A$ as the average time for the \textbf{w/o} model (without splitting) to reach its $F1^H_{w/o}$ (if in an experiment, the highest $F1$ below $F1^H_{w/o}$, the reach time is recorded as $200$). 
Time $B$ is the average time for the \textbf{M1} model to get $F1^H_{w/o}$.
%
The $\Delta_{w/o}$ of \textbf{M1} model is calculated by $A$ minus $B$.
If the value is negative, the \textbf{M1} model can achieve the best prediction earlier than the \textbf{w/o} model.

As shown in table \ref{tab:split_compare}, although \textbf{M3} has a relatively larger $T^H$, it has the best $F1^H$ score on all datasets, 
which is an average $23.7\%$ improvement compared to the \textbf{w/o} model. 
Besides, \textbf{M3} can give the prediction of the same performance nearly $100$ hours earlier.
%
This significant performance difference conveys two observations. 
First, the features fluctuate frequently in the first $200$ hours, thus the segment splitting is indispensable.
%which makes the performance of the \textbf{w/o} model significantly lower than other models. 
Secondly, detecting malicious activities does not necessarily need very late-coming data, 
we can extract the most discriminative information from an earlier segment and achieve more accurate detection of malicious addresses.





==> section/5_6_feat_contri.tex <==
\begin{figure}
	\centering
	\vspace{-0ex}
	\includegraphics[width=.9\columnwidth, angle=0]{image/imp_score_distribution.pdf}
	\vspace{-1ex}
	\caption{Feature importance score evolution and feature constitution for status vectors.}
	\label{fig:hack_status}
	\vspace{-5ex}
\end{figure}
To verify that our model selects features differently for different activities, we plot the importance score over time.
%
First, as shown in Fig.~\ref{fig:hack_status}, we see that the Path feature has high importance scores on all three datasets, which again proves the usefulness of our path feature.
%
In addition, we found that for Hack and Ransomware, the ST-Path feature has a higher contribution than the LT-Path feature.

For the hack, it is generally a criminal who invades the system of an exchange or a large company, steals the private key of its wallet, and then quickly transfers the funds to a secure account through a series of methods such as peeling-chain. Since the fund's source is the exchange with tensive connections with outside, the ST-BK path provides rich temporal and topology information, so ST-BK accounts for the most significant proportion. Secondly, money laundering activities will gradually disperse dirty money so that the transfer-out structural pattern can be well reflected in the ST-FR path.

For ransomware, the source of funds is similar to a Hack. The victims are usually exchanges, or pay ransoms through exchanges, so the weight of ST-BK's path will be higher. Because there will be some time lag for the victim to pay the ransom, the information can usually be reflected by the Address-Features (AF). So the weight of the AF is also relatively high. In addition, since ransomware usually has multiple victims, there will be various addresses accepting the ransom, and each address will aggregate all the ransoms into one total address. Therefore, the weight of LT-FR will be higher.

For darknet, its nature is similar to a trading platform, but due to the concealment, users are required to pay tokens in a specific way, leading to a slightly higher proportion of ST-BK. In addition, because it is a platform, the need for money laundering is not too frequent, so the pattern of LT-FR can help distinguish darknet addresses from other regular addresses.

For importance score evolution, the trend of hack and ransomware will not change much because these two behaviors last for a short time. After completing the task, there will be no further visible activity in these early 200 hours. On the other hand, the darknet will continue to operate and get exposed gradually over time, so the weight of AF will slowly increase.


\begin{figure}
	\centering
	\vspace{-0ex}
	\includegraphics[width=1.\columnwidth, angle=0]{image/Hack_case_decision_Tree.pdf}
	\vspace{-4ex}
	\caption{(a) Status decision tree for hack dataset. 
	         (b) Survival probability of example address. Color are consistent with leaf nodes in status decision tree.
	         (c) Semantic meaning of features in decision tree}
	\label{fig:hack_status}
	\vspace{-2ex}
\end{figure}

==> table/aug_delete_compare.tex <==
\begin{table}[htbp]
    \centering
    \fontsize{10}{11}\selectfont
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \toprule
    \toprule
    &Model & Acc. & Prec. & Rec. & F1^E & F1^C \cr
    \midrule
    \multirow{3}{*}{{H}} &	 w/o     &0.996	        &0.737	     &0.192          &0.303     	 &0.303	\cr
                         &   D	     &\bf{0.997}	&\bf{0.833}	 &0.191	         &0.310	         &0.301	\cr
                         &	 D/A	 &\bf{0.997}	&0.831	     &\bf{0.207}	 &\bf{0.331}	 &\bf{0.323}\cr
    \midrule
    \multirow{3}{*}{{R}} &	 w/o     &0.973     	&0.624   	 &0.220	         &0.309	         &0.290	\cr
                         &   D	     &0.973	        &\bf{0.627}	 &0.220	         &0.318	         &0.281	\cr
                         &	 D/A	 &\bf{0.974}	&0.604	     &\bf{0.290}	 &\bf{0.387}	 &\bf{0.349}\cr
    \midrule
    \multirow{3}{*}{{D}} &	 w/o     &\bf{0.933}	&0.639	     &0.398      	 &0.497	         &0.427\cr
                         &   D	     &0.932	        &\bf{0.640}	 &0.390	         &0.473	         &0.425	\cr
                         &	 D/A	 &0.932	        &0.613	     &\bf{0.455}	 &\bf{0.528}     &\bf{0.470}\cr
    \bottomrule
    \bottomrule
    \end{tabular}
    \vspace{0cm}
    \caption{Scores of different feature filtering schemes. w/o: without feature selection. D: conducting deleting processes only. A: conducting augment processes only. D/A: implementing both deleting and augmenting.}
    \vspace{-0.3cm}
    \label{tab:model_compare}
\end{table}                          






==> table/model_compare_bkup.tex <==
\begin{table*}
    \centering
    \fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
    \caption{Scores of the different prediction models. Evo-PT and Evo-PT (E) are our \emph{Evolve Path Tracer} with/wo ``Early Stop'' mechanism. Underline stands for the best score in the group, Bold stands for the best score in all groups.}
    \vspace{-2ex}
    \begin{tabular}{cccccccccccccccc}
    \toprule
    \multirow{2}{*}{\makecell{{Model}}} 
    & \multicolumn{5}{c}{Hack} & \multicolumn{5}{c}{Ransomware} & \multicolumn{5}{c}{Darknet} \cr
    &$Acc.$ & $Prec.$ & $Rec.$ & $F1^E$ & $F1^C$ & $Acc.$ & $Prec.$ & $Rec.$ & $F1^E$ & $F1^C$ & $Acc.$ & $Prec.$ & $Rec.$ & $F1^E$ & $F1^C$  \cr
    \midrule
    DT     &0.996   &0.247   &0.051   &0.084   &0.084   &0.964   &0.073   &0.014   &0.025   &0.019   &0.908   &0.183   &0.012   &0.020   &0.018\cr
    RF     &0.996   &0.718   &0.134   &0.238   &0.205   &0.964   &0.004   &0.000   &0.000   &0.000   &0.909   &0.468   &0.013   &0.015   &0.016\cr
    XGB    &0.992   &0.081   &0.044   &0.049   &0.048   &0.968   &0.455   &0.421   &0.437   &0.415   &0.913   &0.571   &0.203   &0.291   &0.278\cr
    \midrule
    GCN        &0.736   &0.106   &0.282   &0.163   &0.104   &0.878   &0.223   &0.923   &0.360   &0.359   &0.841   &0.322   &0.813   &0.463   &0.456\cr
    Skip-GCN   &0.651   &0.143   &0.524   &0.226   &0.125   &0.881   &0.226   &0.910   &0.364 	&0.361   &0.780   &0.260   &0.889   &0.400 	 &0.404\cr
    Evo-GCN    &0.760   &0.145   &0.335   &0.196   &0.146   &0.866   &0.200   &0.871   &0.322 	&0.326   &0.737   &0.216   &0.822   &0.342 	 &0.343\cr
    \midrule
    GRU        &0.970   &0.090   &0.499   &0.133   &0.152   &0.901   &0.280   &0.856   &0.389   &0.355   &0.874   &0.518   &0.819   &0.601   &0.438\cr
    M-LSTM     &0.977   &0.113   &0.445   &0.152   &0.183   &0.919   &0.332   &0.870   &0.443   &0.418   &0.880   &0.528   &0.822   &0.612   &0.449\cr
    CED	       &0.980   &0.115   &0.401   &0.154   &0.181   &0.921   &0.329   &0.846   &0.442   &0.415   &0.861   &0.490   &0.835   &0.582   &0.414\cr
    SAFE       &0.974   &0.076   &0.394   &0.133   &0.119   &0.885   &0.246   &0.856   &0.382   &0.294   &0.828   &0.418   &0.865   &0.557   &0.343\cr
    Transformer&0.971   &0.094   &0.464   &0.132   &0.157   &0.928   &0.358   &0.853   &0.467   &0.446   &0.876   &0.515   &0.856   &0.615   &0.438\cr
    \midrule
    Inten-M(Feat)  &0.996   &1.000   &0.274   &0.412   &0.440   &0.986   &0.930   &0.770   &0.797   &0.801   &0.945   &0.851   &0.689   &0.736   &0.624\cr
    Inten-M(+Idx)  &0.997   &1.000   &0.298   &0.436   &0.470   &0.988   &0.889   &0.793   &0.820   &0.824   &0.945   &0.794   &0.766   &0.762   &0.631\cr
    \bottomrule
    \end{tabular}
    \vspace{-3ex}
    \label{tab:sota_compare}
\end{table*}
     

==> table/n_gram_compare.tex <==
\begin{table}
    \centering
    \fontsize{10}{10}\selectfont  
    \begin{tabular}{c|c|c|cccc}
    \toprule
    \toprule
    & Feat. & Clus. & 1-Gram & 2-Gram & 3-Gram & 4-Gram \cr
    \midrule %\rotatebox[origin=c]{90}
    \multirow{4}{*}{H} &\multirow{4}{*}{52} &\multirow{4}{*}{23}        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\\
                                                                        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr                                                                    
    \midrule
    \multirow{4}{*}{R} &\multirow{4}{*}{52} &\multirow{4}{*}{23}        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr  
    \midrule
    \multirow{4}{*}{D} &\multirow{4}{*}{52} &\multirow{4}{*}{23}  &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr
                                                                        &0.056  &0.085  &0.076  &0.076\cr  
    \bottomrule
    \bottomrule
    \end{tabular}
    \vspace{0cm}
    \caption{Scores of different feature combinations on three illicit datasets(H:Hack, R:Ransomware, D: Darknet).}
    \label{tab:feat_compare}
\end{table}



==> table/split_compare.tex <==
\begin{table}
    \caption{Performance of different splitting schemes. (\textbf{w/o}: without splitting, \textbf{M1}: Change-Rate-Based scheme, \textbf{M2}: Fibonacci-Based Scheme, \textbf{M3}: Uniform Scheme)}
    \begin{center}
    \fontsize{10}{11}\selectfont
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    &$Model$ & $F1^H$ & $T^H$ & $\Delta_{w/o}$ & $\Delta_{M1}$ & $\Delta_{M2}$ \cr
    \hline
    \hline
    \multirow{4}{*}{{H}} &	 w/o &0.336 &\bf{27.8} &- &- &-\cr
                         &	 +M1 &0.373 &35.4 &-144.8 &- &-\cr
                         &	 +M2 &0.374 &36.5 &\bf{-145.5} &+1.3   &-\cr
                         &	 +M3 &\bf{0.391} &49.5 &\bf{-145.5} &\bf{-1.8} &\bf{-2.6}\cr


    \hline
    \multirow{4}{*}{{R}} &	 w/o &0.415 &139.3 &- &-      &-\cr
                         &	 +M1 &0.532 &\bf{84.9} &-89.3  &-      &-\cr
                         &	 +M2 &0.564 &106.6 &-96.9 &-32.7 &-\cr
                         &	 +M3 &\bf{0.580} &105.5 &\bf{-99.1} &\bf{-44.7} &\bf{-26.3} \cr                         
    \hline
    \multirow{4}{*}{{D}} &	 w/o &0.563 &186.5 &-       &-      &-\cr
                         &   +M1 &0.589 &\bf{75.2}  &-77.8  &-      &-\cr
                         &	 +M2 &0.624 &157.7 &-106.2 &26.7 &-\cr
                         &	 +M3 &\bf{0.648} &173.6 &\bf{-115.9} &\bf{-37.9} &\bf{-28.7}\cr   
                         
    \hline
    \end{tabular}
    \vspace{-2ex}
    \label{tab:split_compare}
    \end{center}
\end{table}

